Themis: A Network Bandwidth-Aware Collective Scheduling Policy for Distributed Training of DL Models

Distributed training is a solution to reduce DNN training time by splitting the task across multiple NPUs (e.g., GPU/TPU). However, distributed training adds communication overhead between the NPUs in order to synchronize the gradients and/or activation, depending on the parallelization strategy. In next-generation platforms for training at scale, NPUs will be connected through multi-dimensional networks with diverse, heterogeneous bandwidths. This work identifies a looming challenge of keeping all network dimensions busy and maximizing the network BW within the hybrid environment if we leverage scheduling techniques for collective communication on systems today. We propose Themis, a novel collective scheduling scheme that dynamically schedules collectives (divided into chunks) to balance the communication loads across all dimensions, further improving the network BW utilization. Our results show that on average, Themis can improve the network BW utilization of the single All-Reduce by 1.72X (2.70X max), and improve the end-to-end training iteration performance of real workloads such as ResNet-152, GNMT, DLRM, and Transformer-1T by 1.49X (2.25X max), 1.30X (1.78X max), 1.30X (1.77X max), and 1.25X (1.53X max), respectively.

==> algorithms/ThemisFlex.tex <==
\begin{algorithm}[H]
  \caption{\schOpt Algorithm}\label{alg:ThemisFlex}
  \textbf{Inputs:} CollectiveType (CT),  CollectiveSize (CS), ChunksPerCollective (CPC), TotalNPUs (P), Threshold (T)\\
  \textbf{Output:} A 2D list $Schedule[][]$ where $Schedule[i][]$ gives the order of dimensions the i'th chunk should traverse for the collective. 
  \begin{algorithmic}[1]
    \Procedure{Schedule\_Collective}{$CT, CS, CPC$}
      \State DimLoadTracker.initializeToZero()
      \State ChunkSize=CS/CPC
      \While{CS>0} 
        \State currentLoads=DimLoadTracker.getLoads()
        \State minDim=findMinimumLoadDim(currentLoads)
        \State loadDiff=currentLoads.max()-currentLoads.min
        \State size=LatencyModel.getChunkSizeForLoad(
        \State \hspace{110}$minDim,loadDiff$)
        \If {$size< Threshold$}
            \State $Schedule[i][]$=BaselineSchedule(
            \State \hspace{110}$CT, ChunkSize$)
            \State $CS=CS-size$
        \Else
            \If {$CT== All-Reduce$}
                \State $RS\_Sch$=SCHEDULER.SCHEDULE(
                \State \hspace{120}$RS,size$)
                \State $AG\_Sch$=reverseOrder($RS\_Sch$)
                %\State $AG\_Sch$=SCHEDULER.SCHEDULE(
                %\State \hspace{120}$AG,size/P$)
                \State $Schedule[i][]$=concatenate($RS\_Sch$,$AG\_Sch$)
            \Else
                \State $Schedule[i][]$=SCHEDULER.SCHEDULE(
                \State \hspace{135}$CT,size$)
            \EndIf
            \State $CS=CS-size$
        \EndIf
      \EndWhile
      \State \textbf{return} $Schedule$
    \EndProcedure
    \Procedure{Scheduler.Schedule}{$CT, ChunkSize$}\Comment{\textit{Schedules a chunk}}
        \State currentLoads=DimLoadTracker.getLoads()
        \If {$CT== Reduce-Scatter$}
            \State schedule=getIndexOfSortedList(
            \State \hspace{90}$loads,ascending$)
        \Else 
            \If{$CT== All-Gather$}
                \State schedule=getIndexOfSortedList(
                \State \hspace{90}$loads,descending$)
            \EndIf
        \EndIf
        \State newLoad=LatencyModel.calcLoads(
        \State \hspace{90}$chunkSize,schedule,CT$)
        \State DimLoadTracker.update(newLoad)
        \State \textbf{return} schedule
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

==> content/HPCA_comments.tex <==
\section{\red{HPCA Comments}}
\squishlist
    \item \red{it is difficult to get how the basic collective communication algorithm works in the Section 1 and Section 2}
    \item \red{how their proposed algorithm adapt to various types of workloads with more DNNs --- the communication-computation patterns of collective algorithm could vary depending on the characteristics of DNNs}
    \item \red{What is the accuracy of proposed algorithm? In other words, how much the decision of Themis is close to the optimal one in terms of BW utilization?}
    \item \red{It'd be great to see How Themis will adapt to the network variability, e.g., varying bandwidth of connections due to other workloads.}
    \item \red{it'd be helpful to identify the portion of communication in the collective training depending on the various settings including collective size, topology structure, DNN characteristics, batch execution, and so on.}
    \item \red{Build a simple mini cluster of say 4 machines, each with 2 GPUs over NVLink (doesn't have to be the fanciest gpus, just NVLinked to evaluate the network chunck scheduling).}
    \item \red{Does the baseline exactly indicate the multi-rail hierarchical algorithm in [17]? If not, what is the difference between the baseline and the algorithm in 17?}
    \item \red{The discussion on Intra-Dimension Chunk Scheduling in IV-C is not convincing enough. It is advised to add more discussions or justifications.}
    \item \red{There are several assumptions involved in the algorithm design. For example, "Themis assumes the All-Gather schedule is the reverse order of obtained Reduce-Scatter schedule", "we assume the baseline scheme uses a simple FIFO-based intra-dimension chunk execution." These assumptions lay the foundation of the design. However, I wondered whether such assumptions simply the situation reasonably and the situation might be much more complex than the paper assumed.}
    \item \red{It appears that the paper does not discuss the overhead/complexity of the greedy search used in the proposed schedule policy. With the dimension and nodes increasing, the searching will contribute a lot to the overall overhead, it is advised to discuss this part in the paper.}
    \item \red{Why not treat these networks as single-level heterogenous networks instead of hierarchical networks, then use a technique such as Blink to schedule the operations on this heterogenous network?}
    \item \red{On the other hand, how much benefit would you gain if the bandwidth differences between levels was larger? This is more typical if you look at scenarios like intra-node vs. cross-node communication for a GPU cluster}
    \item \red{What exactly is the baseline and does it conform to any state of the art system. For example, MVAPICH 2 GDR seems to already apply some of what you discuss?}
    \item \red{How does your approach compare to prior work that looked at collectives over heterogeneous networks? "Efficient Large Message Broadcast using NCCL and CUDA-Aware MPI for Deep Learning (EuroMPI 2016)", "ECO: Efficient Collective Operations for Communication on Heterogeneous Networks (IPPS 1996)", "Optimizing the steady-state throughput of Broadcasts on heterogeneous platforms (2003)".}
\squishend

==> content/introduction_bckp.tex <==
\section{Introduction}
Deep Neural Networks (DNNs) are constantly growing in demand due to their vast applicability in different areas such as computer vision \cite{ResNet}, language modeling \cite{Transformer}, recommendation systems \cite{DLRM}, etc. In order to improve accuracy and enable emerging applications, the general trend has been towards an increase in both model size and the training dataset \cite{OPENAI}. 
Emerging models have already hit 1 Trillion parameters \cite{Transformer1T}.
This makes training of such DNNs challenging that it might take days or even months if run on a single processing unit. Such long latencies are not acceptable for many real-time DNNs (e.g. recommendation models) that need to be trained constantly using the training samples produced daily. Another factor is that a single compute unit cannot fit the entire model and training data within its limited memory capacity. In this paper, we abstract the compute unit by using the term Neural Processing Unit (NPU). NPUs can be CPU, GPU, TPU, or any other type of accelerator.

Distributed training has been proposed as a solution to overcome the challenges of training large models. In distributed training, the workload is divided across one or multiple dimensions, according to the parallelization strategies, and then distributed across multiple NPUs. The two most famous parallelization strategies are: i) data-parallel, where a mini-batch is split, and ii) model parallel, where a model is divided across NPUs. However, no matter what parallelization strategy is used, the result is the inevitable communication between the NPUs to exchange gradients and/or activations.

\insertFigureNew{CommSizes}{Aggregated collective communication sizes per training iteration for popular DNN models when they are distributed across 1K NPUs.}{0.95}

\insertFigureNew{IntroBWUtil}{\textcolor{blue}{The (training time) speedup vs. average BW utilization for three different-sized Transformer workloads running on six different topologies (please refer to \autoref{sec:motivation} for full description of workloads and topologies). The DNNs are: (i) \transformersmall (17 Billion parameters), (ii) \transformermedium (a.k.a. Transformer-175B, has 175 Billion parameters), and (iii) \transformerlarge (1 Trillion parameters). For each topology, its speedup is normalized to when its BW utilization is 10\%. The bold dots show the baseline BW utilization. }}{0.95}

There are two main methods to handle communication: i) through a centralized parameter server, or ii) using explicit NPU-to-NPU communication to exchange data by using collective communication patterns (e.g., \allreduce. Discussed in detail in \autoref{sec:background}) \cite{astrasim}. In this paper, we focus on the second approach, as it is more scalable and also has lower overhead \cite{CommBottleneck1}.

\textcolor{blue}{As previous studies showed (e.g., \cite{NVidiaSwitch,CommBottleneck1,CommBottleneck2,CommBottleneck3}), communication overhead is becoming an important factor, and in many cases the main bottleneck, in determining the training performance. We identify that increased communication overhead stems from the two main challenges.} 

\textcolor{blue}{\textbf{Challenge 1: Increased Communication Size. }}\autoref{fig:CommSizes} shows how the communication grows, in terms of collective communication operations, for the most popular DNNs in recent years. Such drastic communication growth is primarily due to the orders of magnitude increase in model size (from 60M parameters in ALexNet \cite{AlexNet}, to 1T parameters in transformer1T \cite{Transformer1T}), necessitating distributed training across large number of NPUs to reduce the computation time. However, increasing the communication size and the number of NPUs means increased communication overhead. Thus, large-scale training platforms require efficient network to prevent the communication overhead to become the bottleneck. \textcolor{blue}{This brings us to the second challenge.}

\insertWideFigureNew{DatacenterNetwork}{An example of a distributed training platform with multi-layer interconnection network in datacenters.}{0.95}

\textcolor{blue}{\textbf{Challenge 2: Underutilized Network BW. }}In today's datacenters, for training large models at scale, the NPUs are connected through multi-dimensional interconnection links with different bandwidth and latency. For example, a server blade may be comprised of multiple NPU chips, each chip consists of multiple NPU cores interconnected through a high-BW silicon interposer within the chip (dim1) \cite{HabanaPtP}. The NPU cores within the same server might be then locally connected through the inter-chip links (dim2) \cite{IntelExaScale}. NPUs within the same rack are then connected to the top of the rack (TOR) switch (dim3) using the Network Interface Controller (NIC) connectivity \cite{IntelExaScale,NVIDIASuperPod}. Inter-rack NPU communications are enabled through L1 (dim 4) and L2 (dim5) switches. \autoref{fig:DatacenterNetwork}.a shows the abstraction of a such multi-dimensional network. Note that the NPU connectivity to each dimension could be through dedicated links per each dimension (e.g., torus in \autoref{fig:DatacenterNetwork}.b) or by interconnecting previous dimension switches (e.g., hierarchical switch in \autoref{fig:DatacenterNetwork}.c). In any case, these topologies form separate physical dimensions. 

%commented for MICRO revision
To better utilize the multi-dimensional networks, multi-rail hierarchical collective communication algorithms are proposed (discussed in details in \autoref{sec:background}) \cite{blueconnect}. For example, in the case of \allreduce, communication is pipelined through a series of \reducescatter stages starting from dim1 (first physical dimension) all the way up to dimD (last physical dimension). Then, a series of \allgather stages are performed in the reverse order (i.e. starting from dimD and go back down to dim1). \autoref{fig:DatacenterNetwork}.b and \autoref{fig:DatacenterNetwork}.c show the communication pipeline stages using this method (more details in \autoref{subsec:HierarchicalCollectives}). To utilize all dimensions at the same time, data is broken into chunks and then the chunks are fed (scheduled) into the pipeline in order. However, as we will show in this paper, variable chunk size and network BW results in unbalanced pipeline stage latencies. This means that the overall communication performance is dictated by the slowest stage, making other pipeline stages underutilized, and hence some network dimensions cannot reach their maximum BW utilization.

%This is the shorter version of the above paragraph
%To better utilize the multi-dimensional networks, multi-rail hierarchical collective communication algorithms are proposed (discussed in details in \autoref{sec:background}) \cite{blueconnect} that performs the communication through a series of pipeline stages (for \allreduce, it is a series of Reduce-Scatters followed by series if All-Gathers) operating on different network dimension. \autoref{fig:DatacenterNetwork}.b and \autoref{fig:DatacenterNetwork}.c show the communication pipeline stages using this method for two sample topologies (more details in \autoref{subsec:HierarchicalCollectives}). To utilize all dimensions at the same time, data is broken into chunks and then the chunks are fed (scheduled) into the pipeline in order. However, as we will show in this paper, variable chunk size and network BW results in unbalanced pipeline stage latencies, resulting in BW underutilization.

\textcolor{blue}{\textbf{Putting Everything Together. }To better understand the effect of increased communication size and BW underutilization on the communication overhead, \autoref{fig:IntroBWUtil} shows the overall training time speedup gained as the avg. network BW utilization increases for three different-sized language model DNNs. As \autoref{fig:IntroBWUtil} shows, larger DNNs are more sensitive to networks performance (more details in \autoref{subsec:RealWorkloadResults}). This is because they are mainly communication bound and hence, improvements in network performance results in more overall speeedup. In addition, \autoref{fig:IntroBWUtil} also shows baseline mostly fails to utilize the available BW efficiently due to unbalanced stage latencies. There are some exceptions in the case of \transformermedium where baseline can reach to near full utilization. This is becasue in those workload/topology configurations, the workload only issues collectives that span only one network dimension at a time (partial collective). Hence, unequal stage latencies does not occur. In general, if the ideal utilization (100\%) can be achieved, the training performance on average is improved by 1.06$\times$, 1.07$\times$, and 1.37$\times$ over the baseline for \transformersmall, \transformermedium and \transformerlarge, respectively.}

In this paper, we propose \sch, a novel chunk scheduling scheme that dynamically gives different chunks distinct pipeline schedules to maximize the utilization of all network dimensions. We use the fact that algorithmically there is no strict ordering to perform \reducescatter or \allgather stages. In other words, to perform  \reducescatter/\allgather stages a chunk may start at any network dimension and traverse dimensions in any order. The only synchronization point is that the \reducescatter stages must be completed before starting \allgather. \sch uses this fact and schedules chunks differently to balance loads of all network dimensions.

In short, we make the following contributions:
\squishlist
    \item We identify the problem of unbalanced stage latencies in the baseline methods which rely on the fixed pipeline schedules for all chunks of data to communicate. 
    \item We propose \sch, a novel chunk scheduling scheme for multi-dimensional networks that dynamically schedules the chunks to maximize utilization of each dimension.
    \item We evaluate \sch and compare its performance against the baseline scheduling scheme for both the microbenchmark single collectives and end-to-end training workloads running on representative training platforms in the ASTRA-SIM \cite{astrasim} simulator. Our results show that on average, \sch improves the network communication time by 1.70$\times$ and achieves the BW utilization of 95.22\%. \sch improves the end-to-end training latency for \resnet, \gnmt, and \transformerlarge by 1.16$\times$ (1.29$\times$ max), 1.21$\times$ (1.46$\times$ max), and 1.33$\times$ (1.54$\times$ max), respectively.
    \item Using our analysis of efficient schedulings, we formulate different scenarios regarding the network BW distribution and give insights to the network designers for efficient BW distribution for the multi-dimensional networks tailored for large-scale training.
\squishend


%Commented for MICRO 2021 revision
% The rest of the paper is as follows: \autoref{sec:background} explains collective patterns and the current state of-the-art communication algorithm for the multi-dimensional networks. \autoref{sec:motivation} describes the motivation for our proposed chunk scheduling scheme, \autoref{sec:design} presents \sch in detail, \autoref{sec:methodology} shows our evaluation methodology, \autoref{sec:results} shows our results, and finally  \autoref{sec:conclusion} concludes the paper. 

